Qufinite ZX-calculus: a unified framework of qudit ZX-calculi

ZX-calculus is graphical language for quantum computing which usually focuses on qubits. In this paper, we generalise qubit ZX-calculus to qudit ZX-calculus in any finite dimension by introducing suitable generators, especially a carefully chosen triangle node. As a consequence we obtain a set of rewriting rules which can be seen as a direct generalisation of qubit rules, and a normal form for any qudit vectors. Based on the qudit ZX-calculi, we propose a graphical formalism called qufinite ZX-calculus as a unified framework for all qudit ZX-calculi, which is universal for finite quantum theory due to a normal form for matrix of any finite size. As a result, it would be interesting to give a fine-grained version of the diagrammatic reconstruction of finite quantum theory [Selby2021reconstructing] within the framework of qufinite ZX-calculus.

==> mypackages.tex <==
\usepackage{amsmath, amsthm,amsfonts,amssymb,mathtools,mathdots}

\usepackage{tikz, stmaryrd,tabularx,enumitem}
\usetikzlibrary{shapes}

% theorem styles
%\newtheorem{thm}{Theorem}
%\newtheorem{prop}[thm]{Proposition}
%\newtheorem{lem}[thm]{Lemma}
%\theoremstyle{definition}
%\newtheorem{dfn}[thm]{Definition}
%\newtheorem{axgrp}[thm]{Axioms}
%\theoremstyle{remark}
%\newtheorem{remark}[thm]{Remark}
%\newtheorem{exm}[thm]{Example}
% end theorem styles

% tikz diagrams specification
\usetikzlibrary{arrows, decorations.markings, shapes.geometric, decorations.pathmorphing, decorations.pathreplacing, intersections, patterns,calc, backgrounds}

\pgfdeclarelayer{bg}
\pgfdeclarelayer{mid}
\pgfdeclarelayer{fg}
\pgfsetlayers{bg,mid,fg,main}

\tikzset{
	follow/.style={->, >=stealth, very thick, shorten <=3pt, shorten >=3pt, color=black},%magenta!80},
	edge/.style={line width=.8pt, color=black},
	edgedot/.style={densely dotted, line width=.8pt, color=black},
	edgethdot/.style={densely dotted, line width=.8pt, color=gray},
	edgeth/.style={line width=.8pt, color=gray!60},
	mirror/.style={line width=1.6pt, color=magenta!80},
	dot/.style={circle, draw=black, line width=.8pt, fill=white, inner sep=1.7pt},
	dotth/.style={circle, draw=gray!60, fill=gray!60, inner sep=1.25pt},
	dotwh/.style={circle, draw=gray!60, line width=.8pt, fill=white, inner sep=1.8pt},
	dotwhite/.style={circle, draw=gray, line width=.8pt, fill=white, inner sep=1.8pt},
	dotdark/.style={circle, draw, fill=black, inner sep=1.25pt},
	dotgrey/.style={circle, draw=black, line width=.8pt, fill=gray!60, inner sep=1.6pt},
	coverc/.style={circle, draw=gray, line width=.8pt, inner sep=3pt},
	coverch/.style={circle, draw=gray!30, line width=.8pt, inner sep=3pt},
	%% My definition
	none/.style={circle, draw=none},
	dotred/.style={circle, draw, fill=red, inner sep=1.5pt},
	dotredh/.style={circle, draw, fill=red!60, inner sep=1.5pt},
	dotgreen/.style={circle, draw, fill=green, inner sep=1.5pt},
	dotgreenh/.style={circle, draw, fill=green!60, inner sep=1.5pt},
	boxwhite/.style={rectangle, draw, fill=white, inner sep=3pt},
	boxyellow/.style={rectangle, draw, fill=yellow, inner sep=3pt},
	boxgreen/.style={rectangle, draw, fill=green, inner sep=3pt},
	boxred/.style={rectangle, draw, fill=red, inner sep=3pt},
	uptriyellow/.style={regular polygon,regular polygon sides=3, draw, fill=yellow, inner sep=1.5pt},
	downtriyellow/.style={regular polygon,regular polygon sides=3, draw, fill=yellow, inner sep=1.5pt,rotate=180},
	lefttriyellow/.style={regular polygon,regular polygon sides=3, draw, fill=yellow, inner sep=1.5pt,rotate=90},
	righttriyellow/.style={regular polygon,regular polygon sides=3, draw, fill=yellow, inner sep=1.5pt,rotate=-90},
	%%%%%
	dotthl/.style={circle, draw=gray!60, fill=gray!60, inner sep=0.8pt},
	dotwhl/.style={circle, draw=gray!60, line width=.8pt, fill=white, inner sep=0.8pt},
	dotwhitel/.style={circle, draw=gray, line width=.8pt, fill=white, inner sep=0.8pt},
	dotredl/.style={circle, draw, fill=red, inner sep=0.8pt},
	dotredhl/.style={circle, draw, fill=red!60, inner sep=0.8pt},
	dotgreenl/.style={circle, draw, fill=green, inner sep=0.8pt},
	dotgreenhl/.style={circle, draw, fill=green!60, inner sep=0.8pt},
	boxwhitel/.style={rectangle, draw, fill=white, inner sep=2pt},
	boxyellowl/.style={rectangle, draw, fill=yellow, inner sep=2pt},
	boxgreenl/.style={rectangle, draw, fill=green, inner sep=2pt},
	boxredl/.style={rectangle, draw, fill=red, inner sep=2pt},
	every node/.style={scale=.8},
	every picture/.style={scale=.8},
}
% end tikz diagrams specification

% Specific categories
%\newcommand\cat[1]{\mathbf{#1}}
%\newcommand\graded{\cat{Hilb}^{\mathbb{Z}_2}}

% Other
\newcommand\blankline{\vspace{6pt}}
%\newcommand\comment[1]{\textcolor{magenta}{$^{[\text{#1}]}$}}

%\newcommand\dagg[1]{#1^\dagger}

%\newcommand\braket[2]{\langle\, #1 \,|\, #2 \,\rangle}
%\newcommand\bra[1]{\langle\, #1\,|}
%\newcommand\ket[1]{|\, #1 \, \rangle}
%\newcommand\ketbra[2]{\ket{#1} \! \bra{#2}}
%\newcommand\upto{\underset{\,\diamond}{=}}
%\renewcommand*{\arraystretch}{1.2}

%\linespread{1.05}

